Approximating Sparse PCA from Incomplete Data

We study how well one can recover sparse principal components of a data matrix using a sketch formed from a few of its elements. We show that for a wide class of optimization problems, if the sketch is close (in the spectral norm) to the original data matrix, then one can recover a near optimal solution to the optimization problem by using the sketch. In particular, we use this approach to obtain sparse principal components and show that for \math{m} data points in \math{n} dimensions, \math{O(\epsilon^{-2}\tilde k\max\{m,n\})} elements gives an \math{\epsilon}-additive approximation to the sparse PCA problem (\math{\tilde k} is the stable rank of the data matrix). We demonstrate our algorithms extensively on image, text, biological and financial data. The results show that not only are we able to recover the sparse PCAs from the incomplete data, but by using our sparse sketch, the running time drops by a factor of five or more.

==> experiments_design.tex <==
%

We compute exact PCA and approximate sparse PCA from full data as well as sparse data. For clarity we use following notations to denote various types of principal components we obtain in our experiments. Let $\mathcal{G}$ denote the actual PCs (ground truth) of a given data ($\mathcal{G}$ may not be sparse). 
Let $\mathcal{G}_{\text{max}, r}$ denote the PCs obtained by keeping $r$ largest  components (ranked according to their magnitudes) from $\mathcal{G}$. Thus, $\mathcal{G}_{\text{max}, r}$ is a sparse PC obtained naively from $\mathcal{G}$. $\mathcal{G}_{\text{sp}, r}$ denotes the sparse PC with at most $r$ non-zero components computed via \textit{Spasm} algorithm \cite{KCLE12} on the full data. 
Let $\mathcal{H}_{\text{max}, r}$ denote the naive sparse PCs obtained by keeping $r$ largest components (ranked according to their magnitudes) of PCs of sparsified data whose elements are sampled via hybrid-$(\ell_1,\ell_2)$ sampling. Similarly, $\mathcal{U}_{\text{max}, r}$ denotes the naive sparse PC obtained by keeping $r$ largest components from PCs of sparsified data whose elements are sampled via uniform sampling. 
$\mathcal{H}_{\text{sp}, r}$ and $\mathcal{U}_{\text{sp}, r}$ denote the sparse PCs with at most $r$ non-zero components computed via \textit{Spasm} algorithm on the sparsified data constructed via hybrid-$(\ell_1,\ell_2)$ sampling and uniform sampling, respectively. Table \ref{fig:sparse_PC} summarizes various sparse PCs of full and sparsified data.
%
%  ===============================================
\begin{table}[!h]
\begin{center}
    \begin{tabular}{| l | l | l | l | l | l | l |}
   \hline
& $\mathcal{G}_{\text{max}, r}$& $\mathcal{G}_{\text{sp}, r}$ & $\mathcal{H}_{\text{max}, r}$ 
& $\mathcal{H}_{\text{sp}, r}$  & $\mathcal{U}_{\text{max}, r}$ & $\mathcal{U}_{\text{sp}, r}$  \\ \hline
%
Algo & naive & spasm & naive & spasm & naive & spasm \\ \hline
Data & full & full & sparse & sparse & sparse & sparse \\ \hline
 & - & - & $(\ell_1,\ell_2)$ & $(\ell_1,\ell_2)$ & unif & unif \\ \hline
   \end{tabular}
\caption
{
Summary of various sparse principal components.
}
\label{fig:sparse_PC}
\end{center}
\end{table}
%  ===============================================

\textit{Datasets}\\
\\
We describe various datasets used in our experiments. These datasets span a wide range of application domain, e.g., image, text, stock, and gene expression for cancer.



==> experiments_digit.tex <==
\subsection{Results}\label{experimental_results}
%
Here we report quality of the top sparse principal component for various data. Quality of approximation of other principal components can similarly be derived from the data projected onto the top sparse PCA. 
%
\subsubsection{Handwritten Digit Data}\label{sec:digit}
%
%\textbf{Digit Data}(\cite{Hull94}):
%
We construct incomplete (sparsified) data using $\sim 7\%$ elements from centered data via optimal hybrid sampling ($\alpha^* = 0.42$), as well as, uniform sampling. We construct principal components of such sparsified data via both the naive method and the \textit{Spasm} toolbox. Table \ref{fig:digit_obj_ratio} shows that $f(\mathcal{H}_{\text{max},r})\approx f(\mathcal{G}_{\text{max},r})$ and $f(\mathcal{H}_{\text{sp},r}) \approx f(\mathcal{G}_{\text{sp},r})$ (see Figure  \ref{fig:digit_obj_time}). This indicates that only $7\%$ elements sampled via optimal hybrid sampling preserve the essential structural information of the data irrespective of the choice of algorithm. Moreover, computation of $\mathcal{H}_{\text{max},r}$ and $\mathcal{H}_{\text{sp},r}$ is significantly faster than that of $\mathcal{G}_{\text{max},r}$ and $\mathcal{G}_{\text{sp},r}$ (Table \ref{fig:digit_time_ratio}).
%=============================================
\iffalse % XXXXXXXX  === COMMENTED OUT === XXXXXXXX
\begin{figure}[!ht]
\centering
	\includegraphics[height=3.2cm,width=2.6cm]{results/digit/typical_digits_691_com.png}
	\includegraphics[height=3.6cm,width=5.6cm]{results/digit/SPCA_digit_s5_100_viz.eps}
%	\includegraphics[height=3.2cm,width=5.4cm]{results/digit/digit_heatmap.png}
\caption
{
[Digit data] \textit{(left)} sample digits; \textit{(right)} visualization of top three principal components \textit{without} sparsity constraints: {(left panel)} true PCs of $\matA$, {(middle panel)} PCs of $\matA_{\text{hybrid}}$ using $7\%$ elements of $\matA$, {(right panel)} PCs of $\matA_{\text{unif}}$ using $7\%$ elements of $\matA$. Hybrid sampling shows better quality than uniform sampling.
 %resemblance to true PCs.
}
\label{fig:digit_PC_nosparse}
\end{figure}
\fi
%=============================================
%
% XXXXXXXXXX=========  IGNORE====== XXXXXXXXXXX
\iffalse
\begin{table}[!h]
\begin{center}
    \begin{tabular}{|  c | c || c | c | c | c |}
   \hline
$r$ &  $\frac{s}{m+n}$ & $\frac{f(\mathcal{H}_{\text{max}, r})}{f(\mathcal{G}_{\text{max}, r})}$ 
& $\frac{f(\mathcal{U}_{\text{max}, r})}{f(\mathcal{G}_{\text{max}, r})}$  
& $\frac{f(\mathcal{H}_{\text{sp}, r})}{f(\mathcal{G}_{\text{sp}, r})}$ 
& $\frac{f(\mathcal{U}_{\text{sp}, r})}{f(\mathcal{G}_{\text{sp}, r})}$    \\ \hline \hline  
%---
\multirow{2}{*}{$10$} 
&  5 	& 1.26	&  2.19 	& 0.45	&0.37		\\ \cline{2-6}
&  10 	&  1.11  	& 1.41	& 0.74	&0.50		\\ \cline{2-6}
&  15 	&   1.05 	&  1.25	&0.89		&0.60		\\ \hline
%---
\multirow{2}{*}{$20$} 
&  5 &  1.13  		&   1.43	&0.38		&0.29		\\ \cline{2-6}
&  10 & 1.06		&   1.20	&0.76		&0.37		\\ \cline{2-6}
&  15 & 1.01		&   1.13	&0.89		&0.56		\\ \hline
%---
\multirow{2}{*}{$30$} 
&  5 & 1.02   		&   1.10	&0.5		&0.24		\\ \cline{2-6}
&  10 &1.03		&   1.07	&0.74		&0.44		\\ \cline{2-6}
&  15 &0.98		&   1.04	&0.85		&0.53		\\ \hline
%---
\multirow{2}{*}{$40$} 
&  5 &  1.00  		&  0.94	&0.68		&0.26		\\ \cline{2-6}
&  10 & 1.03		&  1.05	&0.87		&0.62		\\ \cline{2-6}
&  15 & 0.99		&   1.01	&0.90		&0.70		\\ \hline
%---
\multirow{2}{*}{$50$} 
&  5 &  0.99  		& 0.86	&0.77		&0.28		\\ \cline{2-6}
&  10 & 1.01		& 1.01	&0.93		&0.70		\\ \cline{2-6}
&  15 & 0.99		& 0.98	&0.96		&0.76		\\ \hline
%---
\multirow{2}{*}{$60$} 
&  5 &  0.98  		& 0.81	&0.82		&0.33		\\ \cline{2-6}
&  10 & 1.01 		& 0.99	&0.96		&0.77		\\ \cline{2-6}
&  15 &  0.99		& 0.97	&0.98		&0.80		\\ \hline
%---
\multirow{2}{*}{$70$} 
&  5 &  0.97  		& 0.76	&0.87		&0.35		\\ \cline{2-6}
&  10 & 1.00		& 0.96	&0.95		&0.81		\\ \cline{2-6}
&  15 & 0.99		& 0.95  	&0.95		&0.84		\\ \hline
%---
\multirow{2}{*}{$80$} 
&  5 &  0.96  		& 0.72	&0.83		&0.34		\\ \cline{2-6}
&  10 &  0.99		& 0.94	&0.92		&0.77		\\ \cline{2-6}
&  15 & 0.99		& 0.94  	&0.95		&0.81		\\ \hline
%---
\multirow{2}{*}{$90$} 
&  5 &  0.95  		& 0.70	&0.85		&0.37		\\ \cline{2-6}
&  10 & 0.99		& 0.92	&0.94		&0.80		\\ \cline{2-6}
&  15 & 0.99		& 0.94  	&0.96		&0.84		\\ \hline
%---
\multirow{2}{*}{$100$} 
&  5 &  0.96  		& 0.68	&0.89		&0.39		\\ \cline{2-6}
&  10 & 0.99		& 0.92	&0.95		&0.82		\\ \cline{2-6}
&  15 & 0.99		& 0.95  	&0.98		&0.87		\\ \hline
%---
%
   \end{tabular}
\caption{
Sparsification quality $\TNorm{\matA_{pow} - \tilde{\matA}_{pow}}/\TNorm{\matA_{pow}}$  of low-rank `power-law' matrix $\matA_{pow}$ ($k=5$). We compare the quality of hybrid-$(\ell_1,\ell_2)$ sampling and leverage score sampling using two sample sizes. We note (average) $\alpha^*$ of hybrid-$(\ell_1,\ell_2)$ distribution for data $\matA_{pow}$ using $\epsilon=0.05, \delta=0.1$. For $\gamma=0.5, 0.8, 1.0$, we have $\alpha^* = 0.11, 0.72, 0.8$, respectively. 
}
\label{fig:lev_comp_power}
\end{center}
\end{table}
\fi% XXXXXXXXXX======END OF IGNORE====== XXXXXXXXXXX
%  ===============================================
\begin{table}[!h]
\begin{center}
    \begin{tabular}{|  c || c | c | c | c | c |}
   \hline
$r$ & $\frac{f(\mathcal{H}_{\text{max}, r})}{f(\mathcal{G}_{\text{max}, r})}$ 
& $\frac{f(\mathcal{U}_{\text{max}, r})}{f(\mathcal{G}_{\text{max}, r})}$  
& $\frac{f(\mathcal{H}_{\text{sp}, r})}{f(\mathcal{G}_{\text{sp}, r})}$ 
& $\frac{f(\mathcal{U}_{\text{sp}, r})}{f(\mathcal{G}_{\text{sp}, r})}$    \\ \hline \hline  
%---
20	& 1.01		&   1.13	&0.89		&0.56		\\ \hline
%---
40	& 0.99		&   1.01	&0.90		&0.70		\\ \hline
%---
60	&  0.99		& 0.97	&0.98		&0.80		\\ \hline
%---
80	& 0.99		& 0.94  	&0.95		&0.81		\\ \hline
%---
100	& 0.99		& 0.95  	&0.98		&0.87		\\ \hline
%---
   \end{tabular}
\caption{
[Digit data] Comparison of objective values for various sparse principal components.
}
\label{fig:digit_obj_ratio}
\end{center}
\end{table}
%  ===============================================
%  ===============================================
\begin{table}[!h]
\begin{center}
    \begin{tabular}{|  c || c | c | c | c | c |}
   \hline
$r$ & $\frac{t(\mathcal{H}_{\text{max}, r})}{t(\mathcal{G}_{\text{max}, r})}$ 
& $\frac{t(\mathcal{U}_{\text{max}, r})}{t(\mathcal{G}_{\text{max}, r})}$  
& $\frac{t(\mathcal{H}_{\text{sp}, r})}{t(\mathcal{G}_{\text{sp}, r})}$ 
& $\frac{t(\mathcal{U}_{\text{sp}, r})}{t(\mathcal{G}_{\text{sp}, r})}$    \\ \hline \hline  
%---
20	& 23/126	&28/126  	&22/145		&30/145		\\ \hline
%---
40	& 24/129	&27/129 	&20/141		&24/141		\\ \hline
%---
60	& 25/128	&27/128 	&20/136		&23/136		\\ \hline
%---
80	& 25/130	&28/130   	&20/137		&24/137		\\ \hline
%---
100	& 23/124	&29/124   	&20/141		&24/141		\\ \hline
%---
   \end{tabular}
\caption{
[Digit data] Computation time (milliseconds) of various sparse principal components.
}
\label{fig:digit_time_ratio}
\end{center}
\end{table}
%  ===============================================

Figure \ref{fig:digit_obj_time} plots the objective values (divided by the optimal value $f(\mathcal{G})$) for various sparse principal components. We compare $f(\mathcal{G})$ and $f(\mathcal{G}_{\text{sp},r})$ to see that more information is lost due to higher  sparsity (smaller $r$). 
Also, we notice that $f(\mathcal{H}_{\text{sp},r})$ is consistently larger than $f(\mathcal{U}_{\text{sp},r})$ for various sparsity constraints (Table \ref{fig:digit_obj_ratio} and Figure \ref{fig:digit_obj_time}). This indicates the superiority of the optimal hybrid sampling to uniform sampling. However, we notice that $f(\mathcal{U}_{\text{sp},r})$ tends to follow $f(\mathcal{H}_{\text{sp},r})$ (for larger $r$) for this dataset. This is not surprising because a large number of elements of the digit data is either close to $+1$ or $-1$. This is due to the fact that intensity values of each image pixel is normalized in $[-1,+1]$, where presence of intensity is close to $+1$ and lack of it is $-1$.
%
%=============================================
\begin{figure}[!h]
\centering
%	\includegraphics[height=3.5cm,width=4.2cm]{results/digit/SPCA_digit_s5_obj_plus.eps}
%	\includegraphics[height=3.5cm,width=4.1cm]{results/digit/SPCA_digit_s5_time_plus.eps}
\begin{subfigure}[b]{\textwidth}
%	\includegraphics[height=4.0cm,width=8.2cm]{results/digit/SPCA_digit_s5_obj_sp.eps}
	\includegraphics[height=4.0cm,width=8.2cm]{results/digit/SPCA_digit_s5_obj_sp_ratio.eps}
\end{subfigure}
	\includegraphics[height=4.0cm,width=8.2cm]{results/digit/SPCA_digit_s5_time_sp.eps}
\caption
{
[Digit data] (\textit{top figure}) Plot of objective values for various sparse PCA for various sparsity constraints $r$; (\textit{bottom figure}) Plot of computation time (milliseconds) of sparse PCAs for various sparsity constraints $r$. 
%`Sparse hybrid' and `Sparse uniform' indicate the sparsified data obtained from only $\sim 7\%$ elements via optimal hybrid-$(\ell_1,\ell_2)$ sampling and uniform sampling, respectively..
}
\label{fig:digit_obj_time}
\end{figure}
%=============================================
%We plot $\mathcal{E}(\matV_A, \matV_A^{k_0})$, $\mathcal{E}(\matV_A, \matV_\text{hybrid}^{k_0})$, $\mathcal{E}(\matV_A, \matV_\text{unif}^{k_0})$, and $\mathcal{E}(\matV_A^{k_0}, \matV_\text{hybrid}^{k_0})$, $\mathcal{E}(\matV_A^{k_0}, \matV_\text{unif}^{k_0})$.
%=============================================
%\begin{figure}[!h]
%\centering
%	\includegraphics[height=3.5cm,width=4.2cm]{results/digit/SPCA_digit_s5_top10_norm_Vk_diff_plus.eps}
%	\includegraphics[height=3.5cm,width=4.1cm]{results/digit/SPCA_digit_s5_top10_norm_dir_diff_plus.eps}
%%	\includegraphics[height=3.5cm,width=4.2cm]{results/digit/SPCA_digit_s5_ham_Vk_diff.eps}
%%	\includegraphics[height=3.5cm,width=4.1cm]{results/digit/SPCA_digit_s5_ham_dir_diff.eps}
%\caption
%{
%[Digit data] Plot of \textit{relative top norm error} $\mathcal{E}$ for various sparsity constraints $k_0$. (\textit{Left figure}) plot of $\mathcal{E}(\matV_A, \matV_A^{k_0})$ (data actual), $\mathcal{E}(\matV_A, \matV_\text{hybrid}^{k_0})$ (data hybrid), and $\mathcal{E}(\matV_A, \matV_\text{unif}^{k_0})$ (data uniform); (\textit{right figure}) plot of $\mathcal{E}(\matV_A^{k_0}, \matV_\text{hybrid}^{k_0})$ (data hybrid) and $\mathcal{E}(\matV_A^{k_0}, \matV_\text{unif}^{k_0})$ (data uniform).
%}
%\label{fig:digit_topk10_diff}
%\end{figure}
%=============================================
%=============================================
%\begin{figure}[!h]
%\centering
%	\includegraphics[height=3.5cm,width=4.2cm]{results/digit/SPCA_digit_s5_Frob_plus.eps}
%	\includegraphics[height=3.5cm,width=4.1cm]{results/digit/SPCA_digit_s5_proj_diff_plus.eps}
%	\includegraphics[height=3.5cm,width=4.1cm]{results/digit/SPCA_digit_s5_spec_diff_plus.eps}
%\caption
%{
%[Digit data] Quality of projection for various sparsity constraints;  (\textit{top-left figure})  Plot of Frobenius error; (\textit{top-right figure}) Spectral error w.r.t actual, (\textit{bottom figure}) Spectral norm of mutual diff.
%}
%\label{fig:digit_others}
%\end{figure}
%=============================================

Finally, Figure \ref{fig:digit_PC_viz} visualizes the top \textit{three} sparse principal components $\mathcal{G}_{\text{sp},r}$ and $\mathcal{H}_{\text{sp},r}$ for various sparsity constraints $r$. This shows the efficacy of our method producing high-quality  approximation to principal components from incomplete data in a computationally much faster way.
%=============================================
\begin{figure}[!h]
\centering
%
\begin{subfigure}[b]{0.22\textwidth}
%	\includegraphics[height=4.8cm,width=5.5cm]{results/digit/SPCA_digit_s5_100.eps}
	\includegraphics[height=3.6cm,width=3.8cm]{results/digit/SPCA_digit_s5_100.png}
\caption{$r=100\%$}
\end{subfigure}
\begin{subfigure}[b]{0.22\textwidth}
%	\includegraphics[height=4.8cm,width=5.5cm]{results/digit/SPCA_digit_s5_50.eps}
	\includegraphics[height=3.6cm,width=3.8cm]{results/digit/SPCA_digit_s5_50.png}
\caption{$r=50\%$}
\end{subfigure}
\\
\begin{subfigure}[b]{0.22\textwidth}
%	\includegraphics[height=4.8cm,width=5.5cm]{results/digit/SPCA_digit_s5_30.eps}
	\includegraphics[height=3.6cm,width=3.8cm]{results/digit/SPCA_digit_s5_30.png}
\caption{$r=30\%$}
\end{subfigure}
\begin{subfigure}[b]{0.22\textwidth}
%	\includegraphics[height=4.8cm,width=5.5cm]{results/digit/SPCA_digit_s5_10.eps}
	\includegraphics[height=3.6cm,width=3.8cm]{results/digit/SPCA_digit_s5_10.png}
\caption{$r=10\%$}
\end{subfigure}
\caption
{
[Digit data] Visualization of top three sparse principal components $\mathcal{G}_{\text{sp},r}$  and $\mathcal{H}_{\text{sp},r}$ for various sparsity constraints $r$. In each figure, left panel shows $\mathcal{G}_{\text{sp},r}$ and right panel shows $\mathcal{H}_{\text{sp},r}$. Principal components are ordered from top to bottom.
$\mathcal{H}_{\text{sp},r}$ is constructed using $\sim 7\%$ of all data elements sampled via optimal hybrid-$(\ell_1,\ell_2)$ distribution. 
}
\label{fig:digit_PC_viz}
\end{figure}
%=============================================





==> experiments_gene.tex <==
\subsubsection{Gene Expression Data}
%  ===============================================
We sample (and rescale) $\sim 9\%$ elements from centered data via optimal hybrid-$(\ell_1,\ell_2)$ distribution ($\alpha^*=0.92$) and uniform distribution to produce respective sparse sketches.
Table \ref{fig:gene_obj_ratio} shows that $f(\mathcal{H}_{\text{sp},r})$ follows $f(\mathcal{G}_{\text{sp},r})$, and $f(\mathcal{H}_{\text{max},r})$ is reasonably close to $f(\mathcal{G}_{\text{max},r})$. This indicates that only $9\%$ elements sampled via optimal hybrid sampling reasonably preserve the linear structure of this  data irrespective of the choice of algorithm (\textit{`Spasm'} is slightly better). Moreover, computation of $\mathcal{H}_{\text{max},r}$ and $\mathcal{H}_{\text{sp},r}$ is significantly faster than that of $\mathcal{G}_{\text{max},r}$ and $\mathcal{G}_{\text{sp},r}$ (Table \ref{fig:gene_time_ratio}).
%  ===============================================
\begin{table}[!h]
\begin{center}
    \begin{tabular}{|  c || c | c | c | c | c |}
   \hline
$r$ & $\frac{f(\mathcal{H}_{\text{max}, r})}{f(\mathcal{G}_{\text{max}, r})}$ 
& $\frac{f(\mathcal{U}_{\text{max}, r})}{f(\mathcal{G}_{\text{max}, r})}$  
& $\frac{f(\mathcal{H}_{\text{sp}, r})}{f(\mathcal{G}_{\text{sp}, r})}$ 
& $\frac{f(\mathcal{U}_{\text{sp}, r})}{f(\mathcal{G}_{\text{sp}, r})}$    \\ \hline \hline  
%---
20	&0.82 	&0.64   	&0.81		&0.16		\\ \hline
%---
40	&0.82		&0.65   	&0.88		&0.15		\\ \hline
%---
60	&0.83		&0.67 	&0.90		&0.10		\\ \hline
%---
80	&0.84		&0.68   	&0.94		&0.11		\\ \hline
%---
100	&0.84		&0.67   	&0.91		&0.10		\\ \hline
%---
   \end{tabular}
\caption{
[Gene data] Comparison of objective values for various sparse principal components.
}
\label{fig:gene_obj_ratio}
\end{center}
\end{table}
%  ===============================================
%  ===============================================
\begin{table}[!h]
\begin{center}
    \begin{tabular}{|  c || c | c | c | c | c |}
   \hline
$r$ & $\frac{t(\mathcal{H}_{\text{max}, r})}{t(\mathcal{G}_{\text{max}, r})}$ 
& $\frac{t(\mathcal{U}_{\text{max}, r})}{t(\mathcal{G}_{\text{max}, r})}$  
& $\frac{t(\mathcal{H}_{\text{sp}, r})}{t(\mathcal{G}_{\text{sp}, r})}$ 
& $\frac{t(\mathcal{U}_{\text{sp}, r})}{t(\mathcal{G}_{\text{sp}, r})}$    \\ \hline \hline  
%---
20	& 144/512	&183/512  	&136/542		&227/542		\\ \hline
%---
40	& 158/516	&176/516 	&137/548		&245/548		\\ \hline
%---
60	& 147/523	&174/523 	&133/559		&205/559		\\ \hline
%---
80	& 155/544	&183/544   	&143/563		&206/563		\\ \hline
%---
100	& 150/523	&181/523   	&136/557		&202/557		\\ \hline
%---
   \end{tabular}
\caption{
[Gene data] Computation time (milliseconds) of various sparse principal components.
}
\label{fig:gene_time_ratio}
\end{center}
\end{table}
%  ===============================================

Figure \ref{fig:gene_obj_time} plots the objective values (divided by the optimal value $f(\mathcal{G})$) for various sparse principal components. We compare $f(\mathcal{G})$ and $f(\mathcal{G}_{\text{sp},r})$ to see that more information is lost due to higher  sparsity (smaller $r$). 
Also, we notice that $f(\mathcal{H}_{\text{sp},r})$ is significantly larger than $f(\mathcal{U}_{\text{sp},r})$ for various sparsity constraints (Table \ref{fig:gene_obj_ratio} and Figure \ref{fig:gene_obj_time}). This indicates the superiority of the optimal hybrid sampling to uniform sampling. 
%=============================================
\begin{figure}[!h]
\centering
\begin{subfigure}[b]{\textwidth}
%	\includegraphics[height=4.0cm,width=8.2cm]{results/gene/SPCA_gene_s5_obj_sp.eps}
	\includegraphics[height=4.0cm,width=8.2cm]{results/gene/SPCA_gene_s5_obj_sp_ratio.eps}
\end{subfigure}
	\includegraphics[height=4.0cm,width=8.2cm]{results/gene/SPCA_gene_s5_time_sp.eps}
\caption
{
[Gene data] (\textit{top figure}) Plot of objective values for various sparse PCA for various sparsity constraints $r$; (\textit{bottom figure}) Plot of computation time (milliseconds) of sparse PCAs for various sparsity constraints $r$. 
%`Sparse hybrid' and `Sparse uniform' indicate the sparsified data obtained from only $\sim 7\%$ elements via optimal hybrid-$(\ell_1,\ell_2)$ sampling and uniform sampling, respectively.
}
\label{fig:gene_obj_time}
\end{figure}
%=============================================
%=============================================
\iffalse %=== XXXXXXXXXX === COMMENTED OUT ==== XXXXXXXXX
Let $\matA$ be the centered Gene data. We construct incomplete (sparsified) data $\matA_{\text{hybrid}}$ and $\matA_{\text{unif}}$ using $\sim 9\%$ elements from $\matA$ via hybrid sampling and uniform sampling, respectively. 
 Let $\matV_A$ be $n \times 2$ matrix whose columns are the 
top two right singular vectors (principal components) of $\matA$. Let $\matV_A^{k_0}$, 
$\matV_\text{hybrid}^{k_0}$, and $\matV_\text{unif}^{k_0}$ be $n \times 2$ matrices whose 
columns are top two sparse PCs (constrained by $k_0$) of $\matA$, $\matA_\text{hybrid}$, and 
$\matA_\text{unif}$, respectively. 
Figure \ref{fig:gene_obj_time} plots the objective function along with computation time of sparse PCA of $\matA$, $\matA_\text{hybrid}$, and $\matA_\text{unif}$ for Stock data. We see that $\matV_\text{hybrid}^{k_0}$ achieves an objective value close to the value achieved by $\matV_A^{k_0}$ for various $k_0$, while computation time of $\matV_\text{hybrid}^{k_0}$ is significantly faster. Also, $\matV_\text{hybrid}^{k_0}$ achieves much better quality than $\matV_\text{unif}^{k_0}$ despite similar computation time.
%== XXXXXXXXXX === COMMENTED OUT ==== XXXXXXXXX
%=============================================
\begin{figure}[!h]
\centering
%	\includegraphics[height=3.5cm,width=4.2cm]{results/gene/SPCA_gene_s3_obj.eps}
%	\includegraphics[height=3.5cm,width=4.1cm]{results/gene/SPCA_gene_s3_time.eps}
	\includegraphics[height=3.5cm,width=4.2cm]{results/gene/SPCA_gene_s5_obj_plus.eps}
	\includegraphics[height=3.5cm,width=4.1cm]{results/gene/SPCA_gene_s5_time_plus.eps}
\caption
{
[Gene data] (\textit{left figure}) Plot of objective function for various sparsity constraints $k_0$; (\textit{right figure}) Plot of computation time (milliseconds) of sparse PCA for various sparsity constraints $k_0$.
}
\label{fig:gene_obj_time}
\end{figure}
%=============================================
\\
Figure \ref{fig:gene_topk10_diff} plots \textit{relative top norm error} to show how important components of PCs of $\matA_\text{hybrid}$ match that of PCs of $\matA$ for various $k_0$. 
%=============================================
\begin{figure}[!h]
\centering
%	\includegraphics[height=3.5cm,width=4.2cm]{results/gene/SPCA_gene_s3_top10_norm_Vk_diff.eps}
%	\includegraphics[height=3.5cm,width=4.1cm]{results/gene/SPCA_gene_s3_top10_norm_dir_diff.eps}
	\includegraphics[height=3.5cm,width=4.2cm]{results/gene/SPCA_gene_s5_top10_norm_Vk_diff_plus.eps}
	\includegraphics[height=3.5cm,width=4.1cm]{results/gene/SPCA_gene_s5_top10_norm_dir_diff_plus.eps}
\caption
{
Gene Expression data: Plot of difference of top $10\%$ elements for various sparsity constraints; (\textit{left figure})  w.r.t original PCs; (\textit{right figure}) mutual difference.
}
\label{fig:gene_topk10_diff}
\end{figure}
%=============================================
%=============================================
%\begin{figure}[!h]
%\centering
%	\includegraphics[height=3.5cm,width=4.2cm]{results/gene/SPCA_gene_s3_ham_Vk_diff.eps}
%	\includegraphics[height=3.5cm,width=4.1cm]{results/gene/SPCA_gene_s3_ham_dir_diff.eps}
%	\includegraphics[height=3.5cm,width=4.2cm]{results/gene/SPCA_gene_s5_ham_Vk_diff.eps}
%	\includegraphics[height=3.5cm,width=4.1cm]{results/gene/SPCA_gene_s5_ham_dir_diff.eps}
%\caption
%{
%Gene Expression data: Plot of Hamming distance of PCs for various sparsity constraints; (\textit{left figure})  w.r.t original PCs; (\textit{right figure}) mutual difference.
%}
%\label{fig:gene_ham_diff}
%\end{figure}
%== XXXXXXXXXX === END OF COMMENTED OUT ==== XXXXXXXXX%
\fi
%=============================================

We interpret the top features (probes) of the sparse principal components. Table \ref{fig:probe_labels}
 lists the probes corresponding to $r=10$ non-zero components of sparse principal components (we report results only on the top PCA). We notice that most important probes of the actual PCA $\mathcal{G}$ are preserved in $\mathcal{H}_{\text{max}, r}$ and $\mathcal{H}_{\text{sp}, r}$, while $\mathcal{U}_{\text{max}, r}$ and $\mathcal{U}_{\text{sp}, r}$ are arbitrary (Table \ref{fig:probe_labels_ranked}). 
%
%  ===============================================
\begin{table}[!h]
\begin{center}
    \begin{tabular}{| c | l || c | l |}
   \hline
ID & Top probes & ID & Other probes\\ \hline
%
1 & 210081\_at & 11 & 205866\_at \\ \hline
2 & 214387\_x\_at & 12 & 209074\_s\_at \\ \hline
3 & 211735\_x\_at & 13 & 205311\_at \\ \hline
4 & 209875\_s\_at & 14 & 216379\_x\_at \\ \hline
5 & 205982\_x\_at & 15 & 203571\_s\_at \\ \hline
6 & 215454\_x\_at & 16 & 205174\_s\_at \\ \hline
7 & 209613\_s\_at & 17 & 204846\_at \\ \hline
8 & 210096\_at & 18 & 209116\_x\_at \\ \hline
9 & 204712\_at & 19 & 202834\_at \\ \hline
10 & 203980\_at & 20 & 209425\_at \\ \hline
&& 21 & 215356\_at\\ \hline
&& 22 & 221805\_at\\ \hline
&& 23 & 209942\_x\_at\\ \hline
&& 24 & 218450\_at \\ \hline
&& 25 & 202508\_s\_at \\ \hline
   \end{tabular}
\caption
{
[Gene data] List of probes associated with $r=10$ non-zero components of various sparse principal components. IDs are assigned for clarity of comparison.
}
\label{fig:probe_labels}
\end{center}
\end{table}
%  ===============================================
%  ===============================================
\begin{table}[!h]
\begin{center}
    \begin{tabular}{| c | c | c | c | c | c |}
   \hline
$\mathcal{G}_{\text{max}, r}$
& $\mathcal{H}_{\text{max}, r}$ 
& $\mathcal{U}_{\text{max}, r}$ 
& $\mathcal{G}_{\text{sp}, r}$ 
& $\mathcal{H}_{\text{sp}, r}$  
& $\mathcal{U}_{\text{sp}, r}$  \\ 
\hline \hline
%
1  & 4   & 13  & 1	& 4 	& 13 \\ \hline
2  & 1   & 14  & 2	& 1 	& 16 \\ \hline
3  & 11 & 3    & 3 	& 2 	& 15 \\ \hline
4  & 2   & 15  & 4 	& 11 	& 19 \\ \hline
5  & 3   & 5  	& 5 	& 3 	& 20 \\ \hline
6  & 8   & 16  & 6 	& 8 	& 21 \\ \hline
7  & 7   & 6  	& 7 	& 7 	& 22 \\ \hline
8  & 9   & 17  & 8 	& 9 	& 23 \\ \hline
9  & 5   & 4    & 9 	& 5 	& 24 \\ \hline
10 & 12 & 18 & 10 	& 12 	& 25 \\ \hline
   \end{tabular}
\caption
{
[Gene data] Relative ordering of the probes (w.r.t. $\mathcal{G}_{\text{max}, r}$) in $r=10$ non-zero components of various sparse principal components.
}
\label{fig:probe_labels_ranked}
\end{center}
\end{table}
%==========================

Finally, we validate the genes corresponding to the top probes in the context of lung cancer. Table \ref{fig:gene_labels_ranked} lists the top twelve gene symbols in Table \ref{fig:probe_labels}. Also, we note their frequency of occurrence in top ten probes (of their respective principal component) as each gene can be associated with multiple probes.

%\textbf{!!!!!!! ADD VALIDATION SOURCE+EXPLANATION !!!}
%\\
%  ===============================================
\begin{table}[!h]
\begin{center}
    \begin{tabular}{| l | l | l | l | l | l |}
   \hline
$\mathcal{G}_{\text{max}, r}$
& $\nu$ 
& $\mathcal{H}_{\text{max}, r}$ 
& $\nu$
& $\mathcal{H}_{\text{sp}, r}$  
& $\nu$ \\
\hline \hline
%
SFTPC		& 4 	& SFTPC 	& 3 &SFTPC	& 3 \\ \hline
AGER 		& 1 	& SPP1 	& 1 &SPP1	& 1  \\ \hline
SPP 1 		& 1 	& AGER 	& 1 &AGER	& 1  \\ \hline
ADH1B 	& 1 	& FCN3 	& 1 & FCN3 	& 1 \\ \hline
CYP4B1 	& 1 	& CYP4B1 	& 1 &CYP4B1	& 1 \\ \hline
WIF1 		& 1 	& ADH1B 	& 1 &ADH1B	& 1 \\ \hline
FABP4 	& 1 	& WIF1 	& 1 &WIF1	& 1 \\ \hline
		&	& FAM107A 	& 1 &FAM107A& 1 \\ \hline
   \end{tabular}
\caption
{
[Gene data] Gene symbols corresponding to top probes in Table \ref{fig:probe_labels_ranked}. One gene can be associated with multiple probes. Here $\nu$ is the frequency of occurrence of a gene in top ten probes of their respective principal component.
}
\label{fig:gene_labels_ranked}
\end{center}
\end{table}
%  ===============================================
Genes like SFTPC, AGER, WIF1, and FABP4 are known to be down-regulated in lung cancer, while SPP1 is up-regulated. This finding is supported by a functional gene grouping reference: \url{http://www.sabiosciences.com/rt_pcr_product/HTML/PAHS-134Z.html}.
We further perform an enrichment analysis on the set of eight genes for $\mathcal{H}_{\text{max},r}$ and $\mathcal{H}_{\text{sp},r}$ using the tool ToppFun (\url{https://toppgene.cchmc.org/}). Co-expression analysis shows that all eight genes appear in a list of selected probes characterizing non-small-cell lung carcinoma (NSCLC) in \cite{Hou10} (Table S1, $p$-value 9.567$e-13$). Further, six of them (except SPP1 and WIF1) appear in the final list of 187 probe sets that were differentially expressed in NSCLC in \cite{Hou10} (Table S2, $p$-value 1.352$e-12$), while AGER and FAM107A appear in the \textit{top five} highly discriminative genes in \cite{Hou10} (Table S3, $p$-value 1.066$e-6$). 
Additionally, AGER, FCN3, SPP1, and ADH1B appear among the 162 most differentiating genes across two subtypes of NSCLC and normal lung cancer in \cite{Dracheva07} (Supplemental Table 1, $p$-value $1.085e-7$). 
Such findings show how effectively our method can identify important genes that might be responsible for complex diseases like cancer, from only a handful of observed elements. Also, notice that our sampling-based method is able to identify additional important genes, such as, FCN3 and FAM107A in top ten genes.
%  ===============================================
%\begin{table}[!h]
%\begin{center}
%    \begin{tabular}{|  l | l | l |  l | l | l |}
%   \hline
% $\matV_A$ & $f$ &  $\matV_A^{k_0}$ & $f$ &  $\matV_\text{hybrid}^{k_0}$ & $f$ \\ \hline \hline  
%SFTPC & 5 & SFTPC & 5 & SFTPC & 5 \\ \hline
%ADH1B  & 2 & ADH1B & 2 & TMEM100 & 1 \\ \hline
%AGER  & 1 & AGER & 1 & ADH1B & 1 \\ \hline
%SPP1 & 1 & SPP1 & 1 & AGER & 1 \\ \hline
%CYP4B1 & 1 & CYP4B1 & 1 & CYP4B1 & 1 \\ \hline
%WIF1 & 1 & WIF1 & 1 & SPP1 & 1 \\ \hline
%FABP4 & 1 & FABP4 & 1 & FCN3  & 1 \\ \hline
%TMEM100 & 1 & TMEM100 & 1 & WIF1 & 1 \\ \hline
%CLDN18 &1 & ADAM10 & 1 & CLIC5 & 1 \\ \hline
%FCN3 & 1 & SLC39A6 & 1 & CLEC3B & 1 \\ \hline
%CLEC3B & 1 & CLDN18 & 1 & TOP2A & 1 \\ \hline
%FAM107A & 1 & FCN3 & 1 & EDNRB & 1 \\ \hline
%CLIC5 & 1 & CLEC3B & 1 & SEC23A & 1 \\ \hline
%EDNRB & 1 & FAM107A & 1 & FABP4 & 1 \\ \hline
%HBB & 1 & CLIC5 & 1 & LAMP3 & 1 \\ \hline
% &  &  &  & NUP153 & 1 \\ \hline
%  \end{tabular}
%\caption{
%[Gene data] Top twenty components (probes), ranked according to magnitudes, of top two actual PCs and sparse PCs %($k_0=10\%$). There could be multiple genes associated with one probe. Here, $f$ denotes the frequency of occurrence of genes.
%}
%\label{fig:gene_table}
%\end{center}
%\end{table}
%  ===============================================


==> experiments_low_rank.tex <==
\subsection{Sparse PCA of Low-rank Data}
%  ===============================================
We compare optimal hybrid-$(\ell_1,\ell_2)$ sampling with \textit{element-wise leverage score} sampling (similar to \cite{BCSW14}) in the context of producing approximate sparse PCA of data that are explicitly low-rank. Let $\matA$ be a $m \times n$ matrix of rank $\rho$, and its SVD is given by $\matA = \matU\matSig\matV^T$. Then, we define $\mu_i$ (row leverage scores), $\nu_j$ (column leverage scores), and element-wise leverage scores $p_{lev}$ as follows:
\begin{eqnarray*}
%
&& \mu_i = \TNormS{\matU_{(i)}}, \quad \nu_j = \TNormS{\matV_{(j)}},\\ 
&& p_{lev} = \frac{1}{2}\cdot\frac{\mu_i + \nu_j}{(m+n)\rho} + \frac{1}{2mn}, \quad i \in [m], j \in [n]
%
\end{eqnarray*}
%
%for $i=1,...,m$, $j=1,..., n$. 
Element-wise leverage scores of somewhat similar form are used by \cite{BCSW14} in the context of low-rank matrix completion. Note that $p_{lev}$ is a probability distribution on the elements of $\matA$. For a full-rank matrix $\matA$, leverage scores become uniform.  %But our hybrid-$(\ell_1,\ell_2)$ sampling is applicable for general matrices. 
%
We use $p_{lev}$ as a sampling distribution to produce sparse sketches of low-rank data. 

We construct explicit low-rank datasets by projecting the full-rank real datasets onto a low dimensional subspace. We notice that the projected datasets onto the space spanned by top few respective principal components preserve linear structure of the original data. For example, the Digit data show good separation of digits when projected onto the top three principal components. For TechTC and Gene data the top two respective principal components are good enough to form a low-dimensional subspace where the datasets show reasonable separation of two classes of samples. For Stock data we notice a stable rank $\FNormS{\matA}/\TNormS{\matA}$ close to two. For this data we use top three principal components to project the data.

%Let $\mathcal{L}_{\text{max}, r}$ denote the naive sparse PCs obtained by keeping $r$ largest components (ranked according to their magnitudes) of PCs of sparsified data whose elements are sampled via $p_{lev}$ distribution. 
Let, $\mathcal{L}_{\text{sp}, r}$ denote the top sparse PCA with at most $r$ non-zero components computed via \textit{Spasm} toolbox on the sparsified data constructed via sampling according to $p_{lev}$ distribution. 
We use sample size $2\%$, $4\%$, and $2\%$ of all the elements for Digit, TechTC, and Gene data, respectively. For Stock data we sample $2\%$ of the number of non-zero elements.
Figure \ref{fig:ErrorAll_rank_k} compares the objective values $f(\mathcal{H}_{\text{sp}, r})$ and $f(\mathcal{L}_{\text{sp}, r})$, for various low-rank datasets. In all the cases optimal hybrid-$(\ell_1,\ell_2)$ sampling outperforms $p_{lev}$ sampling.

\begin{figure*}
\begin{center}
\begin{tabular}{cccc}
\resizebox{0.24\textwidth}{0.2\textwidth}{\includegraphics{results/digit/SPCA_digit_obj_sp_rank_k2.eps}}&
\resizebox{0.23\textwidth}{0.2\textwidth}{\includegraphics{results/techtc/SPCA_techtc_obj_sp_rank_k2.eps}}
%\\(a) Digits&(b) TectTC\\
\resizebox{0.23\textwidth}{0.2\textwidth}{\includegraphics{results/stock/SPCA_stock_obj_sp_rank_k2.eps}}
&
\resizebox{0.23\textwidth}{0.2\textwidth}{\includegraphics{results/gene/SPCA_gene_obj_sp_rank_k2.eps}}
%\\(c) Stocks&(d) Gene Expression
\end{tabular}
\end{center}
\caption{Performance of sparse PCA for \math{(\ell_1,\ell_2)}-sketch and
leverage sketch over an extensive range for the sparsity constraint \math{r}.
The performance of the leverage sketch is considerably worse
indicating the superiority of \math{(\ell_1,\ell_2)} sampling.
\label{fig:ErrorAll_rank_k}}
\end{figure*}

\iffalse %============== IGNORE ====================
%=============================================
\begin{figure}[!h]
\centering
\begin{subfigure}[b]{0.5\textwidth}
	\includegraphics[height=4.0cm,width=8.2cm]{results/digit/SPCA_digit_obj_sp_rank_k2.eps}
%\caption{Rank-3 Digit data: $\alpha^*=0.21$, and we use sample size $5\cdot (m+n) \approx 2\%$ of all elements.}	
\caption{Rank-3 Digit data: we use sample size $5\cdot (m+n) \approx 2\%$ of all elements. Optimal mixing parameter $\alpha^*=0.21$.}
\end{subfigure}
\begin{subfigure}[b]{0.5\textwidth}
	\includegraphics[height=4.0cm,width=8.2cm]{results/techtc/SPCA_techtc_obj_sp_rank_k2.eps}
\caption{Rank-2 TechTC data: we use sample size $6\cdot (m+n) \approx 4\%$ of all elements.
Optimal mixing parameter $\alpha^*=1$.
}
\end{subfigure}
\begin{subfigure}[b]{0.5\textwidth}
	\includegraphics[height=4.0cm,width=8.2cm]{results/stock/SPCA_stock_obj_sp_rank_k2.eps}
\caption{Rank-3 Stock data: we use sample size $3\cdot (m+n) \approx 2\%$ of number of non-zeros.
Optimal mixing parameter $\alpha^*=0.1$.
}
\end{subfigure}
\begin{subfigure}[b]{0.5\textwidth}
	\includegraphics[height=4.0cm,width=8.2cm]{results/gene/SPCA_gene_obj_sp_rank_k2.eps}
\caption{Rank-2 Gene data: we use sample size $5\cdot (m+n) \approx 5\%$ of all elements.
Optimal mixing parameter $\alpha^*=0.76$.
}
\end{subfigure}
\caption
{
[Low-rank data] 
Plot of objective values for sparse PCA $\mathcal{H}_{\text{sp}, r}$ and $\mathcal{L}_{\text{sp}, r}$ for various sparsity constraints $r$.
}
\label{fig:data_obj_rank_k}
\end{figure}
\fi %============== end of ignore =========================

==> experiments_setup.tex <==
In this section we perform experiments on various data to highlight the preservation of information in incomplete data whose elements are observed via appropriate element-wise sampling methods. We compare the quality of sparse PCA obtained from  incomplete data via various methods described below.

\subsection{Algorithms for Sparse PCA}

We compute exact PCA and approximate sparse PCA from full data, as well as, incomplete (sparse) data. Below we describe various  principal components we obtain in our experiments. Let $\mathcal{G}$ denote the actual PCA's (ground truth) of a given data ($\mathcal{G}$ may not be sparse). 
Let $\mathcal{G}_{\text{max}, r}$ denote the PCA's obtained by keeping $r$ largest  components (ranked according to their magnitudes) from $\mathcal{G}$. Thus, $\mathcal{G}_{\text{max}, r}$ is a sparse PCA obtained naively from $\mathcal{G}$. $\mathcal{G}_{\text{sp}, r}$ denotes the sparse PCA with at most $r$ non-zero components computed using the \textit{Spasm} toolbox of \cite{KCLE12} on the full data. 
Let $\mathcal{H}_{\text{max}, r}$ denote the naive sparse PCA's obtained by keeping the $r$ largest components (ranked according to their magnitudes) of PCA's of sparsified data whose elements are drawn via optimal hybrid-$(\ell_1,\ell_2)$ sampling. Similarly, $\mathcal{U}_{\text{max}, r}$ denotes the naive sparse PCA obtained by keeping the $r$ largest components from PCA's of sparsified data whose elements are drawn via uniform sampling. 
$\mathcal{H}_{\text{sp}, r}$ and $\mathcal{U}_{\text{sp}, r}$ denote the sparse PCA's with at most $r$ non-zero components computed using the \textit{Spasm} toolbox on the sparsified data constructed via optimal hybrid-$(\ell_1,\ell_2)$ sampling and uniform sampling, respectively. Table \ref{fig:sparse_PC} summarizes various sparse PCA's of full and sparsified data.
%
%  ===============================================
\begin{table}[!h]
\begin{center}
\scalebox{0.87}{
    \begin{tabular}{| c || c | c | c | c | c | c |}
   \hline
& $\mathcal{G}_{\text{max}, r}$& $\mathcal{G}_{\text{sp}, r}$ & $\mathcal{H}_{\text{max}, r}$ 
& $\mathcal{H}_{\text{sp}, r}$  & $\mathcal{U}_{\text{max}, r}$ & $\mathcal{U}_{\text{sp}, r}$  \\ \hline \hline
%
Algo & naive & spasm & naive & spasm & naive & spasm \\ \hline
Data & full & full & sparse & sparse & sparse & sparse \\ \hline
$p_{ij}$ & - & - & $(\ell_1,\ell_2)$ & $(\ell_1,\ell_2)$ & unif & unif \\ \hline
   \end{tabular}
}
\caption
{
Summary of various SPCA algorithms.
}
\label{fig:sparse_PC}
\end{center}
\end{table}
%  ===============================================

\subsubsection{Experimental Design}

We measure the quality of approximation of principal components $\matV$ by comparing its objective value to the optimal objective value. Let $f(\matV):= trace(\matV^T\matA^T\matA\matV)$, where $\matA$ is the original centered data. That is, $f(\matV)$ denotes the objective value for $\matV$. 
%We compare the objective values corresponding to various sparse PCs. 
%Comparison between $f(\mathcal{G})$ and $f(\mathcal{G}_{\text{max}, r})$ indicates how much data information we lose due to naive thresholding of actual PCs. 
Comparison between $f(\mathcal{G})$ and $f(\mathcal{G}_{\text{sp}, r})$ tells us how much information is lost due to the sparsity constraint $r$. The difference between $f(\mathcal{G}_{\text{sp},r})$ and $f(\mathcal{G}_{\text{max}, r})$ highlights the importance of a good sparse PCA algorithm. The similarity of $f(\mathcal{G}_{\text{max},r})$ and $f(\mathcal{H}_{\text{max}, r})$, and similarity of $f(\mathcal{G}_{\text{sp},r})$ and $f(\mathcal{H}_{\text{sp}, r})$ measures the preservation of structural information in the original data using only a handful of data elements via element-wise sampling. Finally, comparison between  $f(\mathcal{H}_{\text{sp},r})$ and $f(\mathcal{U}_{\text{sp}, r})$ indicates the importance of appropriate element-wise sampling schemes in order to preserve structural information.
Also, we note the computation time $t(\matV)$, in milliseconds, for various principal components algorithms.


\subsection{Description of Data}

We use real datasets spanning a wide variety of application domain, e.g., image, text, stock, and gene expression for cancer. We  briefly describe the datasets below.
\\
\\
\textbf{Digit Data:}
%
We use a dataset (\cite{Hull94}) of images (300 pixels/inch in 8-bit gray scale) of handwritten digits collected from mails in a working post office. Pixels are treated as features, and pixel values are normalized in $[-1,+1]$. Each $16 \times 16$ digit image is first represented by a column vector by appending the pixels column-wise. Then, we use the transpose of this column vector to form a row in the data matrix. We notice a lot of variation of shapes between digits even in a specific digit class (unlike printed digits) due to wide variety of handwriting styles. We focus on three digits: six (664 samples), nine (644 samples), and one (1005 samples). 
%
This dataset has $m = 2313$ rows and $n=256$ columns.
% shows good separation of three classes of digits when projected onto the space spanned by top three principal components. 
%Therefore, we consider approximating top three PCs using few samples from actual (centered) data. 
\\
\\
\textbf{TechTC Data:}
%
We use a dataset from Technion Repository of Text Categorization Datasets (TechTC) (~\cite{GM04}). The TechTC datasets come from the Open Directory Project (ODP), which is a large, comprehensive directory of the web, maintained by volunteer editors. Each matrix in the TechTC dataset contains a pair of labeled categories from the ODP. The documents are represented in the bag-of-words model, with the words constituting the features of the data. 
%
%We use TechTC datasets (\cite{GM04}). These datasets are bag-of-words model for document-term data describing two topics (ids). 
Our dataset contains 139 documents describing topics with ids 10567 and 11346 (we see the description later in Table \ref{fig:techtc_topic}).
%, and the second one TechTC2 has documents with topic ids 11346 and 22294. 
Rows represent documents and columns are the words. We preprocessed the data by removing all the words of length four or smaller, and then normalized the data to have unit row norm. The dataset is represented by a $139 \times 15170$ matrix.
%The datasets show reasonable separation of two classes of topics when projected onto the space spanned by top two principal components. 
%Therefore, we consider top two PCs to approximate. 
%Table \ref{fig:techtc_table} lists the summary statistics for the TechTC dataset.
%  ===============================================
%\begin{table}[!h]
%\begin{center}
%    \begin{tabular}{|  l | l | l | l|}
%   \hline
% Dimension ($m \times n)$ & \quad $m$ & \quad $n$ & Topics (id1, id2)  \\ \hline \hline  
%\qquad TechTC & \text{ } 139 \quad &  15170 & (10567, 11346)\quad \\ \hline
%%\qquad TechTC2 &  \quad 138 \quad &   11859 \quad \\ \hline
%%\qquad TechTC3 &  \quad 125 \quad &  15485 \quad \\ \hline
%%\qquad TechTC2 &  \text{ } 125 \quad &  14392 & (11346, 22294) \quad \\ \hline
%   \end{tabular}
%\caption{Summary statistics for TechTC dataset.}
%\label{fig:techtc_table}
%\end{center}
%\end{table}
%  ===============================================
%%This is to reduce the bias towards larger documents.\\
%%
%Table \ref{fig:techtc_topic} describes the topics for the TechTC dataset.
%
%============================
\\
\\
\textbf{Stock Data:}
%
We use S\&P100 stock market dataset containing prices of 1218 stocks collected between 1983 and 2011. This temporal dataset has 7056 snapshots of stock prices. We consider stocks as features and each snapshot as a data point describing stock values. Thus, the stock dataset has $m = 7056$ and $n = 1218$. 
%We consider top three PCs to approximate.
%We notice small soft rank $\FNormS{\matX}/\TNormS{\matX}$ of the dataset. 
\\
\\
\textbf{Gene Expression Data:}
%
We use GSE10072 gene expression dataset for lung cancer from the NCBI Gene Expression Omnibus database. The dataset has 107 samples (58 lung tumor cases and 49 normal lung controls). We considered 22,215 probes (features) from the GPL96 platform annotation table to form our $107 \times 22215$ data. 
%We observe that the projection of all samples of the Gene data onto the space spanned by top two PCs  shows good separation between cases and controls. 
%Therefore, we consider approximating top two PCs for this data.



==> experiments_stock.tex <==
\subsubsection{Stock Data}
%
This dataset turns out to be a sparse one. We construct the sparsified data using $\sim 2\%$ of number of non-zero elements from the centered data via optimal hybrid-$(\ell_1,\ell_2)$ sampling $(\alpha^*=0.1)$\footnote{we computed $\alpha^*$ numerically in the range $[0.1, 1]$.}. Also, we have sparse sketch via uniform sampling.
%
Table \ref{fig:stock_obj_ratio} shows that $f(\mathcal{H}_{\text{sp},r})$ follows $f(\mathcal{G}_{\text{sp},r})$, and $f(\mathcal{H}_{\text{max},r})$ is close to $f(\mathcal{G}_{\text{max},r})$. This indicates that only $1\%$ of non-zero elements sampled via optimal hybrid sampling preserve the linear structure of the data irrespective of the choice of algorithm. Moreover, computation of $\mathcal{H}_{\text{sp},r}$ is significantly faster than that of $\mathcal{G}_{\text{sp},r}$ (Table \ref{fig:stock_time_ratio}).
%  ===============================================
\begin{table}[!h]
\begin{center}
    \begin{tabular}{|  c || c | c | c | c | c |}
   \hline
$r$ & $\frac{f(\mathcal{H}_{\text{max}, r})}{f(\mathcal{G}_{\text{max}, r})}$ 
& $\frac{f(\mathcal{U}_{\text{max}, r})}{f(\mathcal{G}_{\text{max}, r})}$  
& $\frac{f(\mathcal{H}_{\text{sp}, r})}{f(\mathcal{G}_{\text{sp}, r})}$ 
& $\frac{f(\mathcal{U}_{\text{sp}, r})}{f(\mathcal{G}_{\text{sp}, r})}$    \\ \hline \hline  
%---
%20	&0.96 	&0.65   	&0.96		&0.64		\\ \hline
20	&1.00 	&0.69   	&1.00		&0.67		\\ \hline
%---
%40	&0.95		&0.63   	&0.96		&0.63		\\ \hline
40	&1.00		&0.66   	&1.00		&0.66		\\ \hline
%---
%60	&0.95		&0.62 	&0.95		&0.62		\\ \hline
60	&0.99		&0.65 	&0.99		&0.66		\\ \hline
%---
%80	&0.95		&0.61   	&0.95		&0.62		\\ \hline
80	&0.99		&0.65   	&0.99		&0.65		\\ \hline
%---
%100	&0.94		&0.61   	&0.95		&0.61		\\ \hline
100	&0.99		&0.64   	&0.99		&0.65		\\ \hline
%---
   \end{tabular}
\caption{
[Stock data] Comparison of objective values for various sparse principal components.
}
\label{fig:stock_obj_ratio}
\end{center}
\end{table}
%  ===============================================
%  ===============================================
\begin{table}[!h]
\begin{center}
    \begin{tabular}{|  c || c | c | c | c | c |}
   \hline
$r$ & $\frac{t(\mathcal{H}_{\text{max}, r})}{t(\mathcal{G}_{\text{max}, r})}$ 
& $\frac{t(\mathcal{U}_{\text{max}, r})}{t(\mathcal{G}_{\text{max}, r})}$  
& $\frac{t(\mathcal{H}_{\text{sp}, r})}{t(\mathcal{G}_{\text{sp}, r})}$ 
& $\frac{t(\mathcal{U}_{\text{sp}, r})}{t(\mathcal{G}_{\text{sp}, r})}$    \\ \hline \hline  
%---
20	& 151/353	&133/353  	&62/467		&40/467		\\ \hline
%---
40	& 151/345	&129/345 	&64/455		&39/455		\\ \hline
%---
60	& 148/346	&133/346 	&61/460		&42/460		\\ \hline
%---
80	& 151/360	&130/360	&66/458		&40/458		\\ \hline
%---
100	& 156/363	&130/363   	&66/447		&41/447		\\ \hline
%---
   \end{tabular}
\caption{
[Stock data] Computation time (milliseconds) of various sparse principal components.
}
\label{fig:stock_time_ratio}
\end{center}
\end{table}
%  ===============================================

Figure \ref{fig:stock_obj_time} plots the objective values (divided by the optimal value $f(\mathcal{G})$) for various sparse principal components. $f(\mathcal{G}_{\text{sp},r})$ and $f(\mathcal{H}_{\text{sp},r})$ appear to achieve near-optimal value even for a small $r$. The reason is similar to TechTC data. This sparse nature of the dataset also explains the poor behavior of uniform sampling in this case.
%
%=============================================
\begin{figure}[!h]
\centering
\begin{subfigure}[b]{\textwidth}
%	\includegraphics[height=4.0cm,width=8.2cm]{results/stock/SPCA_stock_obj_sp.eps}
	\includegraphics[height=4.0cm,width=8.2cm]{results/stock/SPCA_stock_obj_sp_ratio.eps}
\end{subfigure}
	\includegraphics[height=4.0cm,width=8.2cm]{results/stock/SPCA_stock_time_sp.eps}
\caption
{
[Stock data] (\textit{top figure}) Plot of objective values for various sparse PCA for various sparsity constraints $r$; (\textit{bottom figure}) Plot of computation time (milliseconds) of sparse PCAs for various sparsity constraints $r$. 
%`Sparse hybrid' and `Sparse uniform' indicate the sparsified data obtained from only $\sim 7\%$ elements via optimal hybrid-$(\ell_1,\ell_2)$ sampling and uniform sampling, respectively..
}
\label{fig:stock_obj_time}
\end{figure}
%=============================================

\iffalse
%============= COMMENTED OUT =======================
%============= COMMENTED OUT =======================
%============= COMMENTED OUT =======================
%=============================================
%=============================================
\begin{figure}[!h]
\centering
	\includegraphics[height=3.5cm,width=4.2cm]{results/stock/SPCA_stock_s2_obj_plus.eps}
	\includegraphics[height=3.5cm,width=4.1cm]{results/stock/SPCA_stock_s2_time_plus.eps}
\caption
{
[Stock data] (\textit{left figure}) Plot of objective function for various sparsity constraints $k_0$; (\textit{right figure}) Plot of computation time (milliseconds) of sparse PCA for various sparsity constraints $k_0$.
}
\label{fig:stock_obj_time}
\end{figure}
%=============================================
\\
Figure \ref{fig:stock_topk10_diff} plots \textit{relative top norm error} to show how important components of PCs of $\matA_\text{hybrid}$ match that of PCs of $\matA$ for various $k_0$. 
%
%=============================================
\begin{figure}[!h]
\centering
	\includegraphics[height=3.5cm,width=4.2cm]{results/stock/SPCA_stock_s2_top10_norm_Vk_diff_plus.eps}
	\includegraphics[height=3.5cm,width=4.1cm]{results/stock/SPCA_stock_s2_top10_norm_dir_diff_plus.eps}
\caption
{
[Stock data] Plot of \textit{relative top norm error} $\mathcal{E}$ for various sparsity constraints $k_0$. (\textit{Left figure}) plot of $\mathcal{E}(\matV_A, \matV_A^{k_0})$ (data actual), $\mathcal{E}(\matV_A, \matV_\text{hybrid}^{k_0})$ (data hybrid), and $\mathcal{E}(\matV_A, \matV_\text{unif}^{k_0})$ (data uniform); (\textit{right figure}) plot of $\mathcal{E}(\matV_A^{k_0}, \matV_\text{hybrid}^{k_0})$ (data hybrid) and $\mathcal{E}(\matV_A^{k_0}, \matV_\text{unif}^{k_0})$ (data uniform).
}
\label{fig:stock_topk10_diff}
\end{figure}
%=============================================
\fi
%============= END OF COMMENTED OUT =======================
%

%  ===============================================
\begin{table}[!h]
\begin{center}
    \begin{tabular}{| c | l || c | l |}
   \hline
ID & Top stocks & ID & Other stocks\\ \hline
%
1 & T.2 & 11 & HET. \\ \hline
2 & AIG & 12 & ONE.1 \\ \hline
3 & C & 13 & MA \\ \hline
4 & UIS & 14 & XOM \\ \hline
5 & NRTLQ & 15 & PHA.1 \\ \hline
6 & S.1 & 16 & CL \\ \hline
7 & GOOG & 17 & WY \\ \hline
8 & MTLQQ &  &  \\ \hline
9 & ROK &  & \\ \hline
10 & EK &  &  \\ \hline
   \end{tabular}
\caption
{
[Stock data] List of stocks associated with $r=10$ non-zero components of various sparse principal components. IDs are assigned for clarity of comparison.
}
\label{fig:stock_labels}
\end{center}
\end{table}
%  ===============================================
%  ===============================================
\begin{table}[!h]
\begin{center}
    \begin{tabular}{| c | c | c | c | c | c |}
   \hline
$\mathcal{G}_{\text{max}, r}$
& $\mathcal{H}_{\text{max}, r}$ 
& $\mathcal{U}_{\text{max}, r}$ 
& $\mathcal{G}_{\text{sp}, r}$ 
& $\mathcal{H}_{\text{sp}, r}$  
& $\mathcal{U}_{\text{sp}, r}$  \\ 
\hline \hline
%
1 & 1 & 2 & 1 & 1 & 2 \\ \hline
2 & 2 & 11 & 2 & 2 & 11 \\ \hline
3 & 3 & 12 & 3 & 3 & 12 \\ \hline
4 & 4 & 13 & 4 & 4 & 13 \\ \hline
5 & 5 & 14 & 5 & 5 & 14 \\ \hline
6 & 6 & 3 & 6 & 7 & 3 \\ \hline
7 & 7 & 15 & 7 & 6 & 15 \\ \hline
8 & 9 & 9 & 8 & 8 & 9 \\ \hline
9 & 8 & 16 & 9 & 9 & 16 \\ \hline
10 & 11 & 17 & 10 & 11 & 17 \\ \hline
   \end{tabular}
\caption
{
[Stock data]  Relative ordering of the stocks (w.r.t. $\mathcal{G}_{\text{max}, r}$) in $r=10$ non-zero components of various sparse principal components.
}
\label{fig:stock_labels_ranked}
\end{center}
\end{table}
%  ===============================================

%=============================================
%\begin{figure}[!h]
%\centering
%	\includegraphics[height=3.5cm,width=4.2cm]{results/stock/SPCA_stock_s2_ham_Vk_diff.eps}
%	\includegraphics[height=3.5cm,width=4.1cm]{results/stock/SPCA_stock_s2_ham_dir_diff.eps}
%\caption
%{
%Stock data: Hamming distance of PCs. (\textit{left figure}) w.r.t actual PCs (\textit{right figure}) mutual difference.
%}
%\label{fig:stock_ham_diff}
%\end{figure}
%=============================================
%
We interpret the top features (stocks) of the sparse principal components. Table \ref{fig:stock_labels}
 lists the stocks corresponding to $r=10$ non-zero components of sparse principal components (we report results only on the top PCA). 

We notice that most important stocks of the actual PCA $\mathcal{G}$ are preserved in $\mathcal{H}_{\text{max}, r}$ and $\mathcal{H}_{\text{sp}, r}$, while $\mathcal{U}_{\text{max}, r}$ and $\mathcal{U}_{\text{sp}, r}$ are arbitrary (Table \ref{fig:stock_labels_ranked}). 
Clearly, these top stocks correspond to big companies controlling the stock market behavior. 

Finally, we observe the effect of suboptimal $\alpha$ on the quality of approximate solution to sparse principal components. We sample elements via $\ell_1$ distribution, i.e., hybrid sampling with $\alpha=1$, as opposed to $\alpha^*=0.1$. Figure \ref{fig:stock_obj_alpha} shows $f(\mathcal{H}_{\text{sp}, r})$ corresponding to two choices of $\alpha$: $\alpha^*=0.1$ and $\alpha=1$. We observe a drop in quality of approximate sparse PCA for such suboptimal choice of $\alpha$.  
%=============================================
\begin{figure}[!h]
\centering
	\includegraphics[height=4.0cm,width=8.2cm]{results/stock/SPCA_stock_obj_sp_alpha.eps}
\caption
{
[Stock data] Effect of suboptimal $\alpha$ on quality of approximation of sparse principal components. We observe a drop in objective value for PCAs of the data sampled via $\ell_1$ sampling, i.e., hybrid sampling with $\alpha=1$. 
}
\label{fig:stock_obj_alpha}
\end{figure}
%=============================================
%
%  ===============================================
%\begin{table}[!h]
%\begin{center}
%    \begin{tabular}{|  l | l | l |  l | l | l |}
%   \hline
% $\matV_A$ & $f$ &  $\matV_A^{k_0}$ & $f$ &  $\matV_\text{hybrid}^{k_0}$ & $f$ \\ \hline \hline  
%T.2 & 3 & T.2 & 3 & AIG & 3 \\ \hline
%AIG & 3 & AIG & 3 & T.2 & 3 \\ \hline
%GOOG & 2 & GOOG & 2 & GOOG & 2 \\ \hline
%C & 2 & C & 2 & C & 2 \\ \hline
%OXY & 1 & OXY & 1 & IBM & 1 \\ \hline
%APPL & 1 & APPL & 1 & MO & 1 \\ \hline
%MO & 1 & MO & 1 & SO & 1 \\ \hline
%SO & 1 & SO & 1 & CVX & 1 \\ \hline
%CVX & 1 & CVX & 1 & AAPL & 1 \\ \hline
%MA & 1 & MA & 1 & COP & 1 \\ \hline
%BNI & 1 & BNI & 1 & ETR & 1 \\ \hline
%EXC & 1 & EXC & 1 & OXY & 1 \\ \hline
%IBM & 1 & IBM & 1 & AEP & 1 \\ \hline
%ETR & 1 & ETR & 1  & BNI & 1 \\ \hline
%  \end{tabular}
%\caption{
%[Stock data] Top twenty components (stocks), ranked according to magnitudes, of top three actual PCs and sparse PCs %($k_0=10\%$). $f$ denotes the frequency of occurrence $\leq 3$.
%}
%\label{fig:stock_table}
%\end{center}
%\end{table}
%  ===============================================
%


==> experiments_techtc.tex <==
%
\subsubsection{TechTC Data}
%
%
%=============================================
We sample (and rescale) $\sim 5\%$ elements from centered data via optimal hybrid-$(\ell_1,\ell_2)$ distribution ($\alpha^*=1$) and uniform distribution to produce respective sparse sketches.
Table \ref{fig:techtc_obj_ratio} shows that $f(\mathcal{H}_{\text{sp},r})\approx f(\mathcal{G}_{\text{sp},r})$, and $f(\mathcal{H}_{\text{max},r})$ is close to $f(\mathcal{G}_{\text{max},r})$. This indicates that only $5\%$ elements sampled via optimal hybrid sampling preserve the linear structure of the data irrespective of the choice of algorithm (\textit{`Spasm'} is slightly better though). Moreover, computation of $\mathcal{H}_{\text{max},r}$ and $\mathcal{H}_{\text{sp},r}$ is significantly faster than that of $\mathcal{G}_{\text{max},r}$ and $\mathcal{G}_{\text{sp},r}$ (Table \ref{fig:techtc_time_ratio}).
%  ===============================================
\begin{table}[!h]
\begin{center}
    \begin{tabular}{|  c || c | c | c | c | c |}
   \hline
$r$ & $\frac{f(\mathcal{H}_{\text{max}, r})}{f(\mathcal{G}_{\text{max}, r})}$ 
& $\frac{f(\mathcal{U}_{\text{max}, r})}{f(\mathcal{G}_{\text{max}, r})}$  
& $\frac{f(\mathcal{H}_{\text{sp}, r})}{f(\mathcal{G}_{\text{sp}, r})}$ 
& $\frac{f(\mathcal{U}_{\text{sp}, r})}{f(\mathcal{G}_{\text{sp}, r})}$    \\ \hline \hline  
%---
20	&0.94 	&0.43   	&0.98		&0.38		\\ \hline
%---
40	&0.94		&0.41   	&0.99		&0.38		\\ \hline
%---
60	&0.94		&0.40 	&0.99		&0.37		\\ \hline
%---
80	&0.93		&0.39   	&0.99		&0.37		\\ \hline
%---
100	&0.93		&0.38   	&0.99		&0.37		\\ \hline
%---
   \end{tabular}
\caption{
[TechTC data] Comparison of objective values for various sparse principal components.
}
\label{fig:techtc_obj_ratio}
\end{center}
\end{table}
%  ===============================================
%  ===============================================
\begin{table}[!h]
\begin{center}
    \begin{tabular}{|  c || c | c | c | c | c |}
   \hline
$r$ & $\frac{t(\mathcal{H}_{\text{max}, r})}{t(\mathcal{G}_{\text{max}, r})}$ 
& $\frac{t(\mathcal{U}_{\text{max}, r})}{t(\mathcal{G}_{\text{max}, r})}$  
& $\frac{t(\mathcal{H}_{\text{sp}, r})}{t(\mathcal{G}_{\text{sp}, r})}$ 
& $\frac{t(\mathcal{U}_{\text{sp}, r})}{t(\mathcal{G}_{\text{sp}, r})}$    \\ \hline \hline  
%---
20	& 97/483	&98/483  	&89/527		&81/527		\\ \hline
%---
40	& 97/501	&93/501 	&88/554		&84/554		\\ \hline
%---
60	& 93/493	&101/493 	&85/543		&86/543		\\ \hline
%---
80	& 101/501	&105/501   	&89/553		&96/553		\\ \hline
%---
100	& 98/508	&99/508   	&89/557		&94/557		\\ \hline
%---
   \end{tabular}
\caption{
[TechTC data] Computation time (milliseconds) of various sparse principal components.
}
\label{fig:techtc_time_ratio}
\end{center}
\end{table}
%  ===============================================

Figure \ref{fig:techtc_obj_time} plots the objective values (divided by the optimal value $f(\mathcal{G})$) for various sparse principal components. Interestingly, $f(\mathcal{G}_{\text{sp},r})$ and $f(\mathcal{H}_{\text{sp},r})$ appear to achieve near-optimal value even for a small $r$. This is because the dataset looks very `spiky', i.e., all the `energy' is stored in few large components. Consequently, top principal component has only few very large components (such matrices are known as `coherent' in matrix completion literature). Optimal hybrid sampling captures such critical elements of the data. As a result, the small number of large components of PCA's are preserved in sparse principal components, resulting in a near-optimal objective value even for small $r$. This `spiky' nature of the dataset also explains why uniform sampling performs very poorly in this case.
%
%=============================================
\begin{figure}[!h]
\centering
\begin{subfigure}[b]{\textwidth}
%	\includegraphics[height=4.0cm,width=8.2cm]{results/techtc/SPCA_techtc_exp_10567_11346_s3_obj_sp.eps}
	\includegraphics[height=4.0cm,width=8.2cm]{results/techtc/SPCA_techtc_exp_10567_11346_s3_obj_sp_ratio.eps}
\end{subfigure}
	\includegraphics[height=4.0cm,width=8.2cm]{results/techtc/SPCA_techtc_exp_10567_11346_s3_time_sp.eps}
\caption
{
[TechTC data] (\textit{top figure}) Plot of objective values for various sparse PCA for various sparsity constraints $r$; (\textit{bottom figure}) Plot of computation time (milliseconds) of sparse PCAs for various sparsity constraints $r$. 
%`Sparse hybrid' and `Sparse uniform' indicate the sparsified data obtained from only $\sim 7\%$ elements via optimal hybrid-$(\ell_1,\ell_2)$ sampling and uniform sampling, respectively..
}
\label{fig:techtc_obj_time}
\end{figure}
%=============================================

\iffalse
%============= COMMENTED OUT =======================
%============= COMMENTED OUT =======================
%============= COMMENTED OUT =======================
%=============================================
\begin{figure}[!h]
\centering
	\includegraphics[height=3.5cm,width=4.2cm]{results/techtc/SPCA_techtc_exp_10567_11346_s3_obj_plus.eps}
	\includegraphics[height=3.5cm,width=4.1cm]{results/techtc/SPCA_techtc_exp_10567_11346_s3_time_plus.eps}
%	\includegraphics[height=3.5cm,width=4.1cm]{results/techtc/SPCA_techtc_exp_10567_11346_s3_ham_Vk_diff.eps}
%	\includegraphics[height=3.5cm,width=4.1cm]{results/techtc/SPCA_techtc_exp_10567_11346_s3_ham_dir_diff.eps}
\caption
{
[TechTC1 data] (\textit{left figure}) Plot of objective function for various sparsity constraints $k_0$; (\textit{right figure}) Plot of computation time (milliseconds) of sparse PCA for various sparsity constraints $k_0$.
}
\label{fig:techtc1_obj_time}
\end{figure}
%=============================================
%============= COMMENTED OUT =======================
\\
Figures \ref{fig:techtc1_topk10_diff} and \ref{fig:techtc2_topk10_diff} plot \textit{relative top norm error} to show how important components of PCs of $\matA_\text{hybrid}$ match that of PCs of $\matA$ for various $k_0$ for TechTC1 and TechTC2, respectively. 
%
%=============================================
\begin{figure}[!h]
\centering
	\includegraphics[height=3.5cm,width=4.2cm]{results/techtc/SPCA_techtc_exp_10567_11346_s3_top10_norm_Vk_diff_plus.eps}
	\includegraphics[height=3.5cm,width=4.1cm]{results/techtc/SPCA_techtc_exp_10567_11346_s3_top10_norm_dir_diff_plus.eps}
\caption
{
[TechTC1 data] Plot of \textit{relative top norm error} $\mathcal{E}$ for various sparsity constraints $k_0$. (\textit{Left figure}) plot of $\mathcal{E}(\matV_A, \matV_A^{k_0})$ (data actual), $\mathcal{E}(\matV_A, \matV_\text{hybrid}^{k_0})$ (data hybrid), and $\mathcal{E}(\matV_A, \matV_\text{unif}^{k_0})$ (data uniform); (\textit{right figure}) plot of $\mathcal{E}(\matV_A^{k_0}, \matV_\text{hybrid}^{k_0})$ (data hybrid) and $\mathcal{E}(\matV_A^{k_0}, \matV_\text{unif}^{k_0})$ (data uniform).
}
\label{fig:techtc1_topk10_diff}
\end{figure}
%=============================================
%=============================================
%\begin{figure}[!h]
%\centering
%	\includegraphics[height=3.5cm,width=4.2cm]{results/techtc/SPCA_techtc_exp_10567_11346_s3_ham_Vk_diff.eps}
%	\includegraphics[height=3.5cm,width=4.1cm]{results/techtc/SPCA_techtc_exp_10567_11346_s3_ham_dir_diff.eps}
%\caption
%{
%TechTC data 10567:11346: Plot of Hamming distance of PCs for various sparsity constraints; (\textit{left figure})  w.r.t original PCs; (\textit{right figure}) mutual difference.
%}
%\label{fig:techtc1_ham_diff}
%\end{figure}
%=============================================
%============= COMMENTED OUT =======================
%=============================================
\begin{figure}[!h]
\centering
	\includegraphics[height=3.5cm,width=4.1cm]{results/techtc/SPCA_techtc_exp_11346_22294_s3_obj_plus.eps}
	\includegraphics[height=3.5cm,width=4.1cm]{results/techtc/SPCA_techtc_exp_11346_22294_s3_time_plus.eps}
%	\includegraphics[height=3.5cm,width=4.1cm]{results/techtc/SPCA_techtc_exp_11346_22294_s3_ham_Vk_diff.eps}
%	\includegraphics[height=3.5cm,width=4.1cm]{results/techtc/SPCA_techtc_exp_11346_22294_s3_ham_dir_diff.eps}
\caption
{
[TechTC2 data] (\textit{left figure}) Plot of objective function for various sparsity constraints $k_0$; (\textit{right figure}) Plot of computation time (milliseconds) of sparse PCA for various sparsity constraints $k_0$.
}
\label{fig:techtc2_obj_time}
\end{figure}
%=============================================
%=============================================
\begin{figure}[!h]
\centering
	\includegraphics[height=3.5cm,width=4.2cm]{results/techtc/SPCA_techtc_exp_11346_22294_s3_top10_norm_Vk_diff_plus.eps}
	\includegraphics[height=3.5cm,width=4.1cm]{results/techtc/SPCA_techtc_exp_11346_22294_s3_top10_norm_dir_diff_plus.eps}
\caption
{
[TechTC2 data] Plot of \textit{relative top norm error} $\mathcal{E}$ for various sparsity constraints $k_0$. (\textit{Left figure}) plot of $\mathcal{E}(\matV_A, \matV_A^{k_0})$ (data actual), $\mathcal{E}(\matV_A, \matV_\text{hybrid}^{k_0})$ (data hybrid), and $\mathcal{E}(\matV_A, \matV_\text{unif}^{k_0})$ (data uniform); (\textit{right figure}) plot of $\mathcal{E}(\matV_A^{k_0}, \matV_\text{hybrid}^{k_0})$ (data hybrid) and $\mathcal{E}(\matV_A^{k_0}, \matV_\text{unif}^{k_0})$ (data uniform).
}
\label{fig:techtc2_topk10_diff}
\end{figure}
%=============================================
%============= COMMENTED OUT =======================
%%=============================================
%\begin{figure}[!h]
%\centering
%	\includegraphics[height=3.5cm,width=4.2cm]{results/techtc/SPCA_techtc_exp_11346_22294_s3_ham_Vk_diff.eps}
%	\includegraphics[height=3.5cm,width=4.1cm]{results/techtc/SPCA_techtc_exp_11346_22294_s3_ham_dir_diff.eps}
%\caption
%{
%TechTC data 11346:22294: Plot of Hamming distance of PCs for various sparsity constraints; (\textit{left figure})  w.r.t original PCs; (\textit{right figure}) mutual difference.
%}
%\label{fig:techtc2_ham_diff}
%\end{figure}
%=============================================
\fi
%============= END OF COMMENTED OUT =======================
%

Finally, we interpret the top features (words) of the sparse principal components in the context of the topics described by the document samples (Table \ref{fig:techtc_topic}). Table \ref{fig:techtc_words} lists the words corresponding to $r=10$ non-zero components of sparse principal components (we report results only on the top PCA). 
%  ===============================================
\begin{table}[!h]
\begin{center}
    \begin{tabular}{|  c | l | }
   \hline
Topic ID & \qquad Description   \\ \hline \hline  
10567 & US: Indiana: Evansville \\ \hline
11346 & US: Florida \\ \hline
%22294 & Canada: British Columbia: Nanaimo \\ \hline
   \end{tabular}
\caption
{
Description of the topics for TechTC dataset.
}
\label{fig:techtc_topic}
\end{center}
\end{table}
%  ===============================================
%  ===============================================
\begin{table}[!h]
\begin{center}
    \begin{tabular}{| l | l || l | l |}
   \hline
ID & Top words & ID & Other words\\ \hline
%
1 & evansville & 11 & service \\ \hline
2 & florida & 12 & small \\ \hline
3 & south & 13 & frame \\ \hline
4 & miami & 14 & tours \\ \hline
5 & indiana & 15 & faver \\ \hline
6 & information & 16 & transaction \\ \hline
7 & beach & 17 & needs \\ \hline
8 & lauderdale & 18 & commercial \\ \hline
9 & estate & 19 & bullet\\ \hline
10 & spacer & 20 & inlets \\ \hline
& & 21 & producer \\ \hline
   \end{tabular}
\caption
{
[TechTC data] List of words associated with $r=10$ non-zero components of various sparse principal components. IDs are assigned for clarity of comparison.
}
\label{fig:techtc_words}
\end{center}
\end{table}
%  ===============================================

We notice that the most important words of the actual PCA $\mathcal{G}$ are preserved in $\mathcal{H}_{\text{max}, r}$ and $\mathcal{H}_{\text{sp}, r}$, while $\mathcal{U}_{\text{max}, r}$ and $\mathcal{U}_{\text{sp}, r}$ are arbitrary (Table \ref{fig:techtc_words_ranked}). Clearly, these top words summarize the topics described in the documents. 
%  ===============================================
\begin{table}[!h]
\begin{center}
    \begin{tabular}{| c | c | c | c | c | c |}
   \hline
$\mathcal{G}_{\text{max}, r}$
& $\mathcal{H}_{\text{max}, r}$ 
& $\mathcal{U}_{\text{max}, r}$ 
& $\mathcal{G}_{\text{sp}, r}$ 
& $\mathcal{H}_{\text{sp}, r}$  
& $\mathcal{U}_{\text{sp}, r}$  \\ 
\hline \hline
%
1 & 1 & 6 & 1 & 1 & 6 \\ \hline
2 & 2 & 14 & 2 & 2 & 14 \\ \hline
3 & 3 & 15 & 3 & 3 & 15 \\ \hline
4 & 4 & 16 & 4 & 4 & 16 \\ \hline
5 & 5 & 17 & 5 & 5 & 17 \\ \hline
6 & 7 & 7 & 6 & 7 & 7 \\ \hline
7 & 6 & 18 & 7 & 8 & 18 \\ \hline
8 & 8 & 19 & 8 & 6 & 19 \\ \hline
9 & 11 & 20 & 9 & 12 & 20 \\ \hline
10 & 12 & 21 & 13 & 11 & 21 \\ \hline
   \end{tabular}
\caption
{
[TechTC data] Relative ordering of the words (w.r.t. $\mathcal{G}_{\text{max}, r}$) in $r=10$ non-zero components of various sparse principal components.
}
\label{fig:techtc_words_ranked}
\end{center}
\end{table}
%  ===============================================

Therefore, important linear structure of the data, e.g., top principal component, is preserved in only $\sim 5\%$ of the elements sampled via optimal hybrid distribution. Moreover, computation of such high-quality approximation to sparse PCA is significantly fast on sampled data.

\iffalse % ========== XXXXXXXXX COMMENTED OUT XXXXXXXX ========
%  ==============///  TECHTC 2  /// ======================
\begin{table}[!h]
\begin{center}
    \begin{tabular}{| l | l || l | l |}
   \hline
ID & Top words & ID & Other words\\ \hline
%
1 & nanaimo & 11 & image \\ \hline
2 & florida & 12 & theatre \\ \hline
3 & south & 13 & balloon \\ \hline
4 & miami & 14 & yahoo \\ \hline
5 & island & 15 & egroups \\ \hline
6 & vancouver & 16 & email \\ \hline
7 & frame & 17 & messages \\ \hline
8 & estate & 18 & countries \\ \hline
9 & beach & 19 & queenmelanie2000\\ \hline
10 & canada & 20 & paydirect \\ \hline
& & 21 & moments \\ \hline
& & 22 & islam \\ \hline
& & 23 & behalf \\ \hline
   \end{tabular}
\caption
{
[TechTC2 data] List of words associated with top ten non-zero components of various sparse principal components.
}
\label{fig:techtc2_words}
\end{center}
\end{table}
%  ===============================================
%  ===============================================
\begin{table}[!h]
\begin{center}
    \begin{tabular}{| c | c | c | c | c | c |}
   \hline
$\mathcal{G}_{\text{max}, r}$
& $\mathcal{H}_{\text{max}, r}$ 
& $\mathcal{U}_{\text{max}, r}$ 
& $\mathcal{G}_{\text{sp}, r}$ 
& $\mathcal{H}_{\text{sp}, r}$  
& $\mathcal{U}_{\text{sp}, r}$  \\ 
\hline \hline
%
1 & 1 & 14 & 1 & 1 & 14 \\ \hline
2 & 2 & 15 & 2 & 2 & 15 \\ \hline
3 & 3 & 16 & 3 & 3 & 16 \\ \hline
4 & 5 & 17 & 4 & 5 & 17 \\ \hline
5 & 4 & 18 & 5 & 4 & 18 \\ \hline
6 & 6 & 19 & 6 & 8 & 19 \\ \hline
7 & 8 & 20 & 8 & 6 & 20 \\ \hline
8 & 7 & 21 & 7 & 7 & 21 \\ \hline
9 & 11 & 22 & 9 & 11 & 22 \\ \hline
10 & 12 & 23 & 10 & 13 & 23 \\ \hline
   \end{tabular}
\caption
{
[TechTC2 data] Order of the words appear in top ten $(r=10)$ non-zero components of various sparse principal components.
}
\label{fig:techtc2_words_ranked}
\end{center}
\end{table}
%  ===============================================
\fi % ========== XXXXXXXXX END OF COMMENTED OUT XXXXXXXX ========

%  ===============================================
%\begin{table}[!h]
%\begin{center}
%    \begin{tabular}{|  l | l | l |  l | l | l |}
%   \hline
%\qquad $\matV_A$ & $f$ & \quad $\matV_A^{k_0}$ & $f$ & \quad $\matV_\text{hybrid}^{k_0}$ & $f$ \\ \hline \hline  
% evansville & 2 & evansville & 2 & evansville & 2 \\ \hline
% florida & 2 & florida & 2 & florida & 2 \\ \hline
% south & 2 & south & 2 & south & 2 \\ \hline
% spacer & 1 & spacer & 1 & spacer & 1 \\ \hline
% miami & 1 & miami & 1 & miami & 1 \\ \hline
% indiana & 1 & indiana & 1 & indiana & 1 \\ \hline
% information & 1 & information & 1 & beach & 1 \\ \hline
%  \end{tabular}
%\caption{
%[TechTC1 data] Top ten components (words), ranked according to magnitudes, of top two actual PCs and sparse PCs ($k_0=10\%$). 
%Here $f$ denotes the frequency of occurrence $\leq 2$.
%}
%\label{fig:techtc1_words}
%\end{center}
%\end{table}
%  ===============================================
%  ===============================================
%\begin{table}[!h]
%\begin{center}
%    \begin{tabular}{|  l | l | l |  l | l | l |}
%   \hline
%\quad $\matV_A$ & $f$ & \quad $\matV_A^{k_0}$ & $f$ & \quad $\matV_\text{hybrid}^{k_0}$ & $f$ \\ \hline \hline  
% nanaimo & 2 & nanaimo & 2 & nanaimo & 2 \\ \hline
% florida & 2 & florida & 2 & florida & 2 \\ \hline
% south & 2 & south & 2 & south & 2 \\ \hline
% miami & 2 & image & 1 & image & 1 \\ \hline
% image & 1 & pixel & 1 & pixel & 1 \\ \hline
% island & 1 & miami & 1 & single & 1 \\ \hline
%  &  & transparent & 1 & transparent & 1 \\ \hline
%  \end{tabular}
%\caption{
%[TechTC2 data] Top ten components (words), ranked according to magnitudes, of top two actual PCs and sparse PCs ($k_0=10\%$). 
%Here $f$ denotes the frequency of occurrence $\leq 2$.
%}
%\label{fig:techtc2_words}
%\end{center}
%\end{table}
%  ===============================================
%


==> proto_alg1.tex <==
\begin{algorithm}[!t]
\centerline{
\caption{Element-wise Matrix Sparsification }\label{alg:proto_alg1}
}
\begin{algorithmic}[1]
%--------------------------------------------------
\STATE \textbf{Input:} $\matA \in \mathbb{R}^{m \times n}$, sample size $s$.
%\STATE \textbf{Input:} $\matA \in \mathbb{R}^{m \times n}$, $\left\{p_{ij}\right\}_{i,j=1}^{m,n}$ such that $p_{ij} \geq 0$ (for all %$i,j$) and $\sum_{i,j=1}^{m,n} p_{ij}=1$, integer $s > 0$.
%--------------------------------------------------
%\STATE \textbf{Set} $s$ as in eq. (\ref{eqn:opt_s}).
\STATE \textbf{Set} $\tilde{\matA} = \textbf{0}_{m \times n}$.
\STATE \textbf{For} $t = 1\ldots s$ (i.i.d. trials with replacement) 
\STATE \quad Randomly sample pairs of indices $(i_t, j_t) \in [m] \times [n]$ with\\
%
\quad 	$\mathbb{P}\left[ (i_t, j_t) =  (i,j)\right]\ =\ p_{ij}$.
%, where $p_{ij}$ are as in (\ref{eqn:probability}), using $\alpha$ as in (\ref{eqn:opt_alpha}).
%
\STATE \quad $\tilde{\matA}_{ij} = \tilde{\matA}_{ij} + \frac{\matA_{ij}}{s\cdot p_{ij}}$.
%\STATE \textbf{Output:} set of sampled pairs of indices $\Omega = \left\{\left(i_t,j_t\right),t=1\ldots s\right\}$, along with rescaled values $\frac{\matA_{i_t j_t}}{s\cdot p_{i_t j_t}}$.
%\STATE \textbf{Output:} $\Omega = \left\{\left(i_t,j_t\right),t=1\ldots s\right\}$, along with rescaled values $\frac{\matA_{i_t j_t}}%{s\cdot p_{i_t j_t}}$.
%
%\STATE \textbf{Sampling operator:} $\mathcal{S}_{\Omega}: \mathbb{R}^{m \times n}\rightarrow \mathbb{R}^{m \times n}$ with
\STATE \textbf{Output}(sparse): 
%
$\tilde{\matA}$.
%$\mathcal{S}_{\Omega}\left(\matA\right) = \frac{1}{s}\sum_{t=1}^s \frac{\matA_{i_t j_t}}{p_{i_t j_t}} \e_{i_t} \e_{j_t}^T.$
%
\end{algorithmic}
\end{algorithm} 
